Visualization-Aware Sampling for Very Large Databases

Interactive visualizations are crucial in ad hoc data exploration and analysis. However, with the growing number of massive datasets, generating visualizations in interactive timescales is increasingly challenging. One approach for improving the speed of the visualization tool is via data reduction in order to reduce the computational overhead, but at a potential cost in visualization accuracy. Common data reduction techniques, such as uniform and stratified sampling, do not exploit the fact that the sampled tuples will be transformed into a visualization for human consumption. We propose a visualization-aware sampling (VAS) that guarantees high quality visualizations with a small subset of the entire dataset. We validate our method when applied to scatter and map plots for three common visualization goals: regression, density estimation, and clustering. The key to our sampling method's success is in choosing tuples which minimize a visualization-inspired loss function. Our user study confirms that optimizing this loss function correlates strongly with user success in using the resulting visualizations. We also show the NP-hardness of our optimization problem and propose an efficient approximation algorithm. Our experiments show that, compared to previous methods, (i) using the same sample size, VAS improves user's success by up to 35% in various visualization tasks, and (ii) VAS can achieve a required visualization quality up to 400 times faster.

==> README <==

January 11, 2007


IEEEtran.bst is the official BibTeX style for authors of the Institute of
Electrical and Electronics Engineers (IEEE) Transactions journals and
conferences.

It also may have applications for other academic work such as theses and
technical reports. The alphanumeric and natbib variants extend the
applicability of the IEEEtran bibstyle family to the natural sciences
and beyond.

The IEEEtran bibstyle is a very comprehensive BibTeX style which provides
many features beyond the standard BibTeX styles, including full support
for references of online documents, patents, periodicals and standards.
See the provided user manual for detailed usage information.

The latest version of the IEEEtran BibTeX style can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/bibtex/

as well as within IEEE's site:

http://www.ieee.org/

Note that the packages at IEEE's site do not contain the natbib and
alphanumeric variants (e.g., IEEEtranN.bst, etc.) as these are not used
for IEEE related work. These files can be obtained on CTAN.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtran home page at my website:

http://www.michaelshell.org/tex/ieeetran/


Enjoy!

Michael Shell
http://www.michaelshell.org/

*******
Version 1.12 (2007/01/11) changes:

 1. Fixed bug with unwanted comma before "et al." when an entry contained
    more than two author names. Thanks to Pallav Gupta for reporting this.

 2. Fixed bug with anomalous closing quote in tech reports that have a
    type, but without a number or address. Thanks to Mehrdad Mirreza for
    reporting this.

 3. Use braces in \providecommand in begin.bib to better support
    latex2html. TeX style length assignments OK with recent versions
    of latex2html - 1.71 (2002/2/1) or later is strongly recommended.
    Use of the language field still causes trouble with latex2html.
    Thanks to Federico Beffa for reporting this.

 4. Added IEEEtran.bst ID and version comment string to .bbl output.

 5. Provide a \BIBdecl hook that allows the user to execute commands
    just prior to the first entry.

 6. Use default urlstyle (is using url.sty) of "same" rather than rm to
    better work with a wider variety of bibliography styles.

 7. Changed month abbreviations from Sept., July and June to Sep., Jul.,
    and Jun., respectively, as IEEE now does. Thanks to Moritz Borgmann
    for reporting this.

 8. Control entry types should not be considered when calculating longest
    label width.

 9. Added alias www for electronic/online.

10. Updated full and abbreviated journal name string definitions in
    IEEEfull.bib and IEEEabrv.bib.

11. New IEEEtranSA.bst, IEEEtranN.bst, and IEEEtranSN.bst variants for
    alphanumeric citation tags and natbib compatibility.


********************************** Files **********************************

README                 - This file.

IEEEtran_bst_HOWTO.pdf - The user manual.

IEEEtran.bst           - The standard IEEEtran BibTeX style file. For use
                         with IEEE work.

IEEEtranS.bst          - A version of IEEEtran.bst that sorts the entries.
                         Some IEEE conferences/publications may use/allow
                         sorted bibliographies.

IEEEexample.bib        - An example BibTeX database that contains the
                         references shown in the user manual.

IEEEabrv.bib           - String definitions for the abbreviated names of
                         IEEE journals. (For use with IEEE work.)
                         
IEEEfull.bib           - String definitions for the full names of IEEE
                         journals. (Do not use for IEEE work.)


Carried on CTAN only, for non-IEEE related work:

IEEEtranSA.bst         - Like IEEEtranS.bst, but with alphanumeric citation
                         tags like alpha.bst. Not for normal IEEE use.

EEEtranN.bst          - Like IEEEtran.bst, but based on plainnat.bst and
                         is compatible with Patrick W. Daly's natbib
                         package. Not for normal IEEE use.

IEEEtranSN.bst         - Sorting version of IEEEtranN.bst. Not for normal
                         IEEE use

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran_bst_HOWTO.pdf, IEEEtran.bst, IEEEtranS.bst,
                   IEEEtranSA.bst, IEEEtranN.bst, IEEEtranSN.bst,
                   IEEEexample.bib, IEEEabrv.bib, IEEEfull.bib
                   
***************************************************************************


==> mip.tex <==
\section{MIP Formulation}
\label{sec:apdx_mip}


In order to find an exact solution to Max Cover Sampling (MCS), we can covert the
problem to an instance of mixed integer programming. The mixed integer 
programming is a constrained version of linear programming in which some
of variables should be one of predefined integer values. The problem of MCS
can be expressed as follows:
\begin{align*}
    \min \quad
    &\sum_{i,j \in [1, N], \atop i < j} \exp(-c \cdot d_{ij}) \cdot b_{ij} \\
    \text{s.t.}\quad
    & \sum_{i \in [1, N]} a_i = K, \quad
    b_{ij} = a_i \cdot a_j, \quad
    a_i, b_{ij} \in \{0, 1\}
\end{align*}
where $N$ is the dataset cardinality, and $a_i$ indicates $x_i$ is chosen. The
above problem is not yet \emph{linear} because it contains multiplication in its
constraints. Therefore, to solve the problem using any toolkit for MIP, we
should linearize the problem.

Note that since both $a_i$ and $b_{ij}$ are binary variables in the above
problem, we can think $b_{ij} = a_i \text{ AND } a_j$. It is known that we
can convert the logical AND operation to the following equivalent expression for
integer programming:
\begin{align*}
    & b_{ij} \le a_i \\
    & b_{ij} \le a_j \\
    & b_{ij} \ge a_i + a_j - 1 \\
    & b_{ij} \ge 0
\end{align*}

Using the above relationship, now we can convert the above problem to the
following one that can be consumed by a MIP toolkit such as GLPK:
\begin{align*}
    \min \quad
    &\sum_{i,j \in [1, N], \atop i < j} \exp(-c \cdot d_{ij}) \cdot b_{ij} \\
    \text{s.t.}\quad
    & \sum_{i \in [1, N]} a_i = K, \quad
    a_i, b_{ij} \in \{0, 1\} \\
    & b_{ij} \le a_i, \quad
    b_{ij} \le a_j, \quad
    b_{ij} \ge a_i + a_j - 1, \quad
    b_{ij} \ge 0
\end{align*}

With the above ILP formulation, we can apply existing approaches to ILP
problems, and the obtained solution is optimal. The solution obtained by solving
this ILP problem has minimal loss, and can be applied when $N$ is very small,
say less than 100. When dataset is of size of interest, however, it is not a
tractable approach.






\ignore{
In order to find an exact solution to Max Cover Sampling (MCS), we can convert the
problem to an instance of mixed integer programming (MIP). The mixed integer 
programming is a constrained version of linear programming in which some
of the variables should be one of the predefined integer values. The problem of MCS
can be converted to an MIP as follows:
\begin{align*}
    \min \quad
    &\sum_{i,j \in [1, N], \atop i < j} \exp(-c \cdot d_{ij}) \cdot b_{ij} \\
    \text{s.t.}\quad
    & \sum_{i \in [1, N]} a_i = K, \quad
    a_i, b_{ij} \in \{0, 1\} \\
    & b_{ij} \le a_i, \quad
    b_{ij} \le a_j, \quad
    b_{ij} \ge a_i + a_j - 1, \quad
    b_{ij} \ge 0
\end{align*}
where $N$ is the dataset cardinality, $a_i$ indicates $x_i$ is chosen, and
$b_{ij}$ indicates both $a_i$ and $a_j$ are chosen. For
more detailed steps on the derivation, please refer to the supplementary
material~\cite{park2014vldbsupp}.
}


==> np_hard.tex <==
\section{Hardness of VAS}
\label{sec:nphard}

In this section, we prove the NP-hardness of \vas~under the condition that the
kernel function $\tilde{\kappa}(s_i,s_j)$ can have any arbitrary value, which is
true in a general setting. One can argue that, however, in practice, $x_i$'s are
enough to be defined in a metric space in which triangular inequality must hold, so
the values of the kernel functions should retain related property. To address
the question, we conduct empirical study in Section~\ref{sec:exp} with Mixed
Integer Programming toolkit to directly solve the problem. The result of the
emprical study also supports our claim.

\begin{theorem}
\vas~(Problem~\ref{prob:vas}) is NP-hard.
\end{theorem}

\begin{proof}
We show the NP-hardness of Problem~\ref{prob:vas} by reducing
\emph{maximum edge subgraph} problem to \vas.

\begin{lemma}
(\emph{Maximum Edge Subgraph}) Given a undirected weighted graph $G = (V, E)$,
choose a subgraph $G' = (V', E')$ with $|V'| = K$ that maximizes
\[
    \sum_{(u,v) \subset E'} w(u,v)
\]
This problem is called \emph{maximum edge subgraph}, and is
NP-hard~\cite{feige2001dense}.
\end{lemma}

To reduce the above problem to \vas, the following procedure is performed: map
$i$-th vertex $v_i$ to $i$-th instance $x_i$, and set the value of
$\tilde{\kappa}(x_i,x_j)$ to $w_{max} - w(v_i, v_j)$, where $w_{max} =
\max_{v_i, v_j \subset V'} w(v_i, v_j)$. The reduction process takes $O(|E| +
|V|)$. Once the set of data points that minimize $\sum_{s_i,s_j \in X}
\tilde{\kappa}(s_i,s_j)$ is obtained by solving \vas, we choose a set of
corresponding vertices, and return as an answer to the \emph{maximum edge
subgraph} problem.  Since the \emph{maximum edge subgraph} problem is NP-hard,
and the reduction process takes a polynomial time, \vas~is also NP-hard.
\end{proof}


==> osm.tex <==
\subsection{OpenStreetMap Data Experiment}
\label{sec:osm}

OpenStreetMap dataset contains 9 years of GPS traces uploaded to OpenStreeMap
project by individuals, and we obtained the dataset from its
repository.\footnote{http://planet.openstreetmap.org/gps/}. We extracted from
the data the GPS logs that contained altitude or elevation record together with a
pair of latitude and longitude. We processed raw {\tt xml} files, and it took more
than a day to extract all the fields into a more condensed {\tt csv} file. 
The total number of the records we extracted
from the dataset was 2,195,899,509, and the size of the extracted {\tt csv} file was
59G on disk.

Figure~\ref{fig:osm_speed} reports the time it took to process the data by
various sampling methods. The sample sizes range from 1K to 1M, and it took
about 1,100 mins for VAS to process the entire dataset to obtain a sample of 1M
records. Notably, due to the large size of the dataset, the sample speed was not
different as much as the experiments with the Geolife dataset.


\input{fig_osm_speed}

For comparison purpose, we generated several scatter plots into image files, and
show them in Figure~\ref{fig:intro:complete}. The first figure
is a scatter plot we obtain by processing 25\% of the entire dataset. The 25\%
of the dataset was the limit we could process using the {\tt pyplot} library on a machine
with 244G memory. Also, generating the plot took huge amount of time. For reading a
dataset from disk and parsing, it took 49 minutes, and for rendering the loaded
data into a scatter plot took more than 4 hours. See that the visualization time
only for 25\% of the data took 4 hours, and this indicates that it will take
possible more than 10 hours for visualization of the entire dataset, if memory
allows. This indicates that when the dataset is massive, sampling-based
visualization will be much more appealing.

Figure~\ref{fig:intro:complete}d is a scatter plot generated
by processing only 10K records. Despite its tiny sample size compared to the
original dataset ($5 \times 10^{-8}\%$),
the figure visualizes many interesting areas that were missed
by other sampling methods in Figure~\ref{fig:intro:complete}b and c. Certainly,
it we zoom into a particular area, we need to use samples with more records to
display rich information. However, at least, this example shows that the high
quality of the scatter plot generated by VAS.

\begin{figure}[h]
	\centering

    \begin{subfigure}[t]{0.4\textwidth}
        \centering
        \includegraphics[width=0.8\textwidth,height=0.6\textwidth]{figs/open_quarter.png}
        \caption{25\% of the original 2B tuple dataset}
    \end{subfigure}
    ~
    \begin{subfigure}[t]{0.4\textwidth}
        \centering
        \includegraphics[width=0.8\textwidth,height=0.6\textwidth]{figs/open_rs_10K.png}
        \caption{A 10K tuple random sample}
    \end{subfigure}

    \vspace{2mm}

    \begin{subfigure}[t]{0.4\textwidth}
        \centering
        \includegraphics[width=0.8\textwidth,height=0.6\textwidth]{figs/open_ss_10K.png}
        \caption{A 10K tuple stratified sample}
    \end{subfigure}
    ~
    \begin{subfigure}[t]{0.4\textwidth}
        \centering
        \includegraphics[width=0.8\textwidth,height=0.6\textwidth]{figs/open_subs_10K.png}
        \caption{A 10K tuple \vas\ sample}
    \end{subfigure}

    \caption{25\% of the original OpenStreetMap dataset and samples of 10K data points.}
    \label{fig:intro:complete}
\end{figure}



==> splom_var.tex <==
\subsection{More Results on Sample Variance Comparison}
\label{sec:splom_var}

\input{fig_variance}

We report both the mean and median of log-variance-ratios introduced in
Section~\ref{sec:corr} for two datasets (Geolife and SPLOM). See
Figure~\ref{fig:variance:appendix}. The X-axis of the plot shows the ratio of
the size of the samples we obtained relative to the original dataset, and the
Y-axis shows the loss function we used. Therefore, the lower the better.

Due to some extreme quantities that appear in calculating the sample variance
using Monte Carlo technique, there is a large gap between our method and the
other sampling methods. To avoid the skewness of those sample variance
computations, we also included median graphs for comparison. Note that in the
graphs, because the Y-axis measures the log value of the variance-ratio, the
difference of 1 indicates a quality difference of 10 times. In all cases, the
samples by our method achieved much lower sample variances, and the gap was
bigger when the sample sizes were small. (This is natural because if the sample
ratio is 1, there should not be any quality difference.)



==> submodular.tex <==
\section{Submodularity of VAS}
\label{sec:sub}

Here, we show that \vas~has the property called \emph{submodularity}. The
property helps us provide a worst-case bound for the approximate algorithm that
will be presented in the following section. Although the wost-case bound is
interesting in a theoretical perspective, the approximate algorithm seems to
create samples whose qualities are quite close to those of optimal samples
according to our empirical study in Section~\ref{sec:runtime_comp}.

Before showing the submodularity of \vas, we first introduce the definition of
submodularity.

\begin{mydef}
(Submodularity) A real-valued function $f$ defined over subsets of a dataset
$D$ is \emph{submodular} if for all $S\subseteq T \subseteq D$ and all $x_i \in
D - T$, $f$ has the following property:
\[
f(S \cup \{x_i\}) - f(S) \ge f(T \cup \{x_i\}) - f(T)
\]
\end{mydef}

The intuitive interpretation of the submodularity is that the gain of adding a new
element $x_i$ to an existing set decreases as the size of the set increases. To
show the submodularity of the problem, we formulate a variant of the problem
that returns the same answer as follows:
\begin{align}
    S = \argmax_{S \subseteq D;\; |S| = K}
    \sum_{s_i, s_j \in S;\; i < j} 1 - \tilde{\kappa}(s_i, s_j)
    \label{eq:subprob}
\end{align}
where we assume that the maximal value of $\tilde{\kappa}(\cdot, \cdot)$ is 1,
which is the condition that can be easily met by normalization.


\begin{lemma}
Let $f(S) = \sum_{s_i, s_j \in S; \; i < j} (1 - \tilde{\kappa}(s_i, s_j))$,
then the function $f$ is submodular.
\label{lemma:sub}
\end{lemma}

\begin{proof}
Let $S \subseteq T \subseteq D$. $f(S \cup \{x\}) - f(S) = \sum_{s_i \in
S} (1 - \tilde{\kappa}(x, s_i))$, and $f(T \cup \{x\}) - f(T) = \sum_{s_i \in T}
(1 - \tilde{\kappa}(x, s_i))$. Then
\begin{align*}
    & \left(f(T \cup \{x\}\right) - f(T))
    - \left(f(S \cup \{x\}) - f(S)\right) \\
    &= \sum_{s_i \in T - S} (1 - \tilde{\kappa}(x, s_i)) \ge 0
\end{align*}
since $\tilde{\kappa}(\cdot, \cdot) \le 1$.
\end{proof}


==> tab_ilp.tex <==
\centering

\scriptsize

\begin{tabular}{|c|c|c|c|c|c|}
\hline
                      &$N$ & Random & ILP  & Greedy & Interchange  \\ \Xhline{2\arrayrulewidth}
\multirow{3}{*}{loss} & 20 & 2.11   & 1.13 & 1.13   & 1.17         \\
                      & 30 & 4.43   & 0.11 & 0.12   & 0.12         \\
                      & 40 & 2.15   & 0.07 & 0.10   & 0.09         \\ \hline
\multirow{3}{*}{\pbox{2cm}{runtime}}
                      & 20 & 0      & 0.13 secs  & 0   &  0        \\
                      & 30 & 0      & 162 secs   & 0   &  0        \\
                      & 40 & 0      & 56.2k secs & 0   &  0        \\ \hline
\end{tabular}





==> tab_user.tex <==
\centering

\scriptsize

\begin{tabular}{|l|r|r|r|}
\hline
Type of Question        & Random & Stratified  & MCS    \\ \Xhline{2\arrayrulewidth}
value estimation        & 50\%   & 55\%        & {\bf 92\%}   \\ 
%density estimation      & {\bf 100\%}  & 50\%        & 62\%   \\ 
preference over methods & 3.4\%  & 10.3\%      & {\bf 86.2\%} \\ \hline
\end{tabular}





==> tab_viz_online.tex <==
\begin{table}[t]
\centering
\small

\begin{subfigure}[b]{0.5\textwidth}
\centering
\begin{tabular}{|l|r|r|r|}
\hline
Method          & Offline   & Online    & Sample Variance \\ \hline
No Sampling     & 0s        & 3m 32s    & 0.0752    \\
Uniform Random  & 1m 11s    & 0.344s    & inf       \\
Stratified      & 4m 22s    & 0.364s    & inf       \\
VAS             & 20m 15s   & 0.384s    & 0.944     \\ \hline
\end{tabular}
\caption{Sample size: 10K}
\end{subfigure}

\vspace{4mm}

\begin{subfigure}[b]{0.5\textwidth}
\centering
\begin{tabular}{|l|r|r|r|}
\hline
Method          & Offline   & Online    & Sample Variance \\ \hline
No Sampling     & 0s        & 3m 32s    & 0.0752    \\
Uniform Random  & 1m 6s     & 1.2s      & inf       \\
Stratified      & 3m 27s    & 1.2s      & 4.20E+53  \\
VAS             & 62m 40s   & 1.2s      & 0.155     \\ \hline
\end{tabular}
\caption{Sample size: 100K}
\end{subfigure}

\caption{Offline and online time required to visualize a scatter plot and the
quality of the samples. VAS took longer offline processing times, but it brought
significant quality gains over other sampling methods. `No Sampling' did not
meet the interactive response time. Geolife was used for dataset, and MathGL was
used to measure the visualization latency.}
\label{tab:viz_online}
\end{table}


==> var_user.tex <==
\subsection{Correlation between Sample Variance and User Success Ratio}
\label{sec:var_user}

Figure~\ref{fig:var_user} depicts the negative correlation bewteen the sample
variance and user success ratio in the regression task. Each dot in the figure
is obtained by averaging the the fraction of the correct answers submitted by
40 unique Turkers on 6 questions. Because the X-axis of the figure is loss
function we aim to minize to obtain a good sample, the negative correlation
bewteen the two metrics shows the validity of our problem formulation.

\input{fig_var_user}

